RichDreamer: A Generalizable Normal-Depth Diffusion Model for Detail Richness in Text-to-3D

Lifting 2D diffusion for 3D generation is a challenging problem due to the lack of geometric prior and the complex entanglement of materials and lighting in natural images. Existing methods have shown promise by first creating the geometry through score-distillation sampling (SDS) applied to rendered surface normals, followed by appearance modeling. However, relying on a 2D RGB diffusion model to optimize surface normals is suboptimal due to the distribution discrepancy between natural images and normals maps, leading to instability in optimization. In this paper, recognizing that the normal and depth information effectively describe scene geometry and be automatically estimated from images, we propose to learn a generalizable Normal-Depth diffusion model for 3D generation. We achieve this by training on the large-scale LAION dataset together with the generalizable image-to-depth and normal prior models. In an attempt to alleviate the mixed illumination effects in the generated materials, we introduce an albedo diffusion model to impose data-driven constraints on the albedo component. Our experiments show that when integrated into existing text-to-3D pipelines, our models significantly enhance the detail richness, achieving state-of-the-art results. Our project page is https://aigc3d.github.io/richdreamer/.

==> 4_method_old.tex <==
\newcommand{\point}{\mathbf{x}}
\newcommand{\dir}{\mathbf{d}}
\newcommand{\pointcolor}{\mathbf{c}}
\newcommand{\density}{\sigma}
\newcommand{\raycolor}{\hat{\mathbf{C}}}
\newcommand{\ray}{\mathbf{r}}
\newcommand{\nerffun}{\mathbf{f}}
\newcommand{\nerfparam}{\phi}

\newcommand{\data}{x}
\newcommand{\latent}{z}
\newcommand{\noise}{\epsilon}
\newcommand{\dmparam}{\theta}
\newcommand{\albedo}{a}
\newcommand{\dmparamalbedo}{\theta_\albedo}
\newcommand{\camera}{c}
\newcommand{\depth}{d}
\newcommand{\dmtime}{t}
\newcommand{\image}{x}
\newcommand{\volumerender}{g}
\newcommand{\prompt}{y}
\newcommand{\encoder}{\mathcal{E}}

\newcommand{\real}{\mathbb{R}}
\newcommand{\diffuse}{k_d}
\newcommand{\roughness}{k_r}
\newcommand{\metallic}{k_m}
\newcommand{\ntangent}{k_n}
\newcommand{\mlpmaterial}{f_\parammat}
\newcommand{\parammat}{\psi}


\section{Method}
%In this section, we detail our approach for text-to-3D generation. 
%Our approach for text-to-3D generation follows a two-stage decoupled generation strategy, where we first generate the geometry of the 3D content, followed by the stage of appearance modeling.
In this section, we introduce a Normal-Depth diffusion model and an Albedo diffusion model to push forward the decoupled 3D generation pipeline, where the geometry is first generated followed by the appearance modeling (see \fref{fig:pipeline}).

\paragraph{Overview}
The existing approach for decoupled generation \cite{chen2023fantasia3d} adopts a text-to-image diffusion model (\ie, Stable-Diffusion \cite{rombach2022high}) to optimize the rendered surface normals of the object for geometry generation. 
However, this direct application is suboptimal due to the discrepancy in data distribution between natural images and normal maps, often leading to unstable optimization and compromised geometric fidelity \cite{chen2023fantasia3d}. 
As a result, appropriate geometry initialization (\eg, 3D ellipsoids with different shapes and orientations, or coarse 3D models) is often needed to achieve good results for different prompts.
In response, we propose to learn a 3D-aware diffusion model tailored for 3D geometry generation. Specifically, we introduce a normal-depth diffusion model pre-trained on an extensive real-world dataset and further fine-tuned on a synthetic dataset, to offer consistent guidance for geometry generation.

Another critical issue in text-to-3D generation is the inaccurate appearance modeling, where materials intermingle with the lighting effects like shadows and specular highlights, often resulting in imprecise relighting. 
In an attempt to address this, our method integrates an albedo diffusion model to regularize the albedo component of the materials, effectively separating the albedo from the influence of lighting artifacts.

\subsection{Normal-Depth Diffusion Model}
To endow the diffusion model with 3D geometric priors for 3D generation tasks, we introduce a novel normal-depth diffusion model.
Different from existing methods that either learn a normal or a depth diffusion model \cite{huang2023humannorm,stan2023ldm3d}, our model captures the joint distribution of normal and depth, leveraging their intrinsic complementary nature-depths describe the macrostructure of the scene while normals provide local surface details. 

\paragraph{Model Architecture}
We adapted the architecture of the publicly available text-to-image diffusion model, Stable Diffusion (SD) \cite{rombach2022high}, with minor modifications.
SD incorporates a variational auto-encoder (VAE) with KL-regularization \cite{kingma2013auto}, and a latent diffusion model (LDM). 
The VAE maps an image of size $512\times 512$ to and from a latent space of size $64\times 64$, and the LDM is a UNet denoiser that learns to denoise the latent feature guided by the text prompt.

For our purpose, we extended the input and output channel number of SD's VAE from three to four channels to encompass three for normals and one for depth, keeping other components unchanged. 
We 

\paragraph{Pre-training on Real-world Data}
The LAION-2B dataset, comprising billions of correlated image and text pairs, served as our foundational training resource \cite{schuhmann2022laion}. 
We prepared our training set with text prompts paired with corresponding normal and depth maps, utilizing Midas-3.1 \cite{ranftl2020towards}, a leading method for monocular depth and normal estimation.

We first trained the Normal-Depth VAE to learn the joint distribution of normal and depth with the MSE reconstruction loss, adversarial loss, and the KL-regularization loss \cite{rombach2022high,esser2021taming}.
We then trained the LDM to enable text to Normal-Depth generation. Denoting $\data$ as the normal and depth data, $\encoder$ the encoder, $z$ the latent feature, and $\noise_{\dmparam}$ the UNet denoiser, the objective for training LDM can be written as:
\begin{align}
    \mathcal{L}_{\text{LDM}} = \mathbb{E}_{\latent\sim \mathcal{E}(\data), \prompt, \dmtime, \noise \sim \mathcal{N}(0,1)}\left[\|\noise_{\dmparam}(\latent_\dmtime, \prompt, \dmtime) - \noise\|^2_2\right],
\end{align}
where $\latent_\dmtime$ is the noised latent variable at a specific denoising timestep $\dmtime$, 
and $\prompt$ the text embedding obtained from the CLIP model \cite{radford2021learning}.
Our results show that the pre-training on the real-world dataset is crucial to maintain the generalization ability on diverse prompts.


\paragraph{Fine-tuning on Synthetic 3D Data}
To enhance object-level 3D generation, we fine-tuned our Normal-Depth LDM on the Objaverse dataset \cite{deitke2023objaverse}, which features ground-truth 3D models. 
We render the ground-truth normal and depth maps with the provided object. 
In the fine-tuning stage, we employed a four-view diffusion technique proposed by MVDream \cite{shi2023mvdream}. The camera poses are mapped by a simple Multilayer Perceptron (MLP) to be the camera embeddings, which will be added to the time embedding to be accessed by the diffusion model.
The training objective in the fine-tune stage is:
\begin{align}
    \mathcal{L}_{\text{LDM}}^{\text{FT}} = \mathbb{E}_{\latent, \prompt, \camera, \dmtime, \noise \sim \mathcal{N}(0,1)}\left[\|\noise_{\dmparam}(\latent_\dmtime, \prompt, \camera, \dmtime) - \noise\|^2_2\right],
\end{align}
where $c$ is the camera condition.

\paragraph{Implementation Details}
For training on the LAION dataset, we follow the data filtering strategy used in the training of SD v2.1 to ensure high-quality data selection. 
The image is resized to $384\times 384$ as input to Midas for estimating normal and depth. \todo{normalization of disparity} 
We initialize the parameters of our model with the pre-trained weights of SD 2.1, with the extra parameters randomly initialized\todo{}.
The computational expense for training the Normal-Depth VAE and LDM amounted to $1,344$ and $11,520$ GPU hours respectively on A100-80G GPUs.

For fine-tuning on the Objaverse dataset, for each 3D object, we established camera positions within a radial distance of 1.4 to 2.0 units and an elevation angle spanning 5 to 30 degrees. We rendered 24 views per object, distributed uniformly across azimuth angles. To enhance the dataset quality, we discarded objects whose rendered images scored low in relevance to the object names as determined by CLIP scores, resulting in a pool of 270,000 training objects. The text prompts used in training were obtained by a hybrid approach: 30\% stemmed from object tags and names, and the remaining 70\% were from Cap3D \cite{luo2023scalable}.
\todo{disparity normalization for the synthetic dataset}
The fine-tuning utilized a batch size of $512$ with gradient accumulation performed every $8$ batches.
This was conducted on 8 GPUs for one week, reaching a total of $20,000$ iterations.

\subsection{Albedo Diffusion Model}
The physically-based rendering (PBR) material model is defined by two principal components: the diffuse component, which is influenced by the albedo, and the specular component, governed by metallic and roughness parameters \cite{burley2012physically}. Ideally, a prior model for appearance modeling should effectively regulate both these components. However, a significant obstacle arises due to the varied creation methods of existing 3D models, leading to a lack of standardization \cite{deitke2023objaverse}. This diversity makes it particularly challenging to acquire a comprehensive dataset with consistent, accurate ground-truth information for the specular component (metallic and roughness properties). 
In light of this difficulty, we introduce an albedo diffusion model to decouple the albedo from complex lighting effects, serving as a preliminary approach to mitigate the challenge of mixed illumination. 


\paragraph{Depth-Conditioned Albedo Generation}
A direct solution for the albedo diffusion model involves fine-tuning a text-to-image diffusion model using paired data of text prompts and albedo maps. 
While this method is effective for sampling, it falls short for 3D generation due to potential misalignments between the generated albedo and the geometry.
Although such a model works well for sampling purposes, it is not suitable for 3D generation as the generated albedo might not aligned with the geometry.
To ensure alignment of generated albedo maps with geometry, we employ the depth map from the corresponding viewpoint as a condition within the albedo Latent Diffusion Model (LDM).
Specifically, we concatenate the depth map with the latent features to serve as input for the UNet denoiser \cite{ramesh2021zero}.

We fine-tune the SD 2.1 on the Objaverse dataset \cite{deitke2023objaverse} to capture the albedo distribution, with the following training objective for the albedo diffusion model:
\begin{align}
    \mathcal{L}_{\text{Albedo}} = \mathbb{E}_{\latent^\albedo, \prompt, \camera, \dmtime, \noise \sim \mathcal{N}(0,1)}\left[\|\noise_{\dmparamalbedo}(\latent^\albedo_\dmtime, \prompt, \camera, \depth, \dmtime) - \noise\|^2_2\right],
\end{align}
where $\latent^\albedo$ represents the latent feature of the albedo map, and $\depth$ is the depth condition.

\subsection{Text-to-3D Generation}

\paragraph{Score Distillation Sampling (SDS)}
Existing 2D lifting approaches for text-to-3D typically employ either a NeRF representation \cite{mildenhall2020nerf,poole2022dreamfusion} or the hybrid DMTet representation \cite{shen2021deep,lin2023magic3d} to represent the 3D content.
Denoting $\nerfparam$ as the parameters of a 3D representation and $\volumerender$ as the differentiable rendering function, the rendered image can be expressed as $\image=\volumerender(\nerfparam)$.
DreamFusion \cite{poole2022dreamfusion} introduces a Score Distillation Sampling (SDS) process that leverages gradient-based score functions to guide the optimization of parameters in 3D representation for object generation:
\begin{equation}
    \label{eq:sds}
    \nabla_{\nerfparam} \mathcal{L}_{\text{SDS}}(\phi, \image=\volumerender(\nerfparam)) = \mathbb{E}_{\dmtime, \noise}\left[w(t)(\noise_{\dmparam}(\latent_\dmtime ; \prompt, \dmtime) - \noise) \frac{\partial \image}{\partial \nerfparam}\right],
\end{equation}
where the expression $(\noise_{\dmparam}(\latent_t; \prompt, t) - \noise)$ represents the difference between the actual noise $\noise$ and the noise estimated by the UNet $\noise_{\dmparam}$. The term $w(t)$ is a weighting term that dependents on the timestep $t$, and $\prompt$ indicates the text embedding.

\paragraph{Geometry Generation}
Our Normal-Depth diffusion model provide additional supervision for the geometry optimization of both NeRF and DMTet representations.

For the DMTet representation, we integrate our Normal-Depth diffusion model into the coarse-to-fine geometry generation process of Fantasia3D \cite{chen2023fantasia3d}.
The normal and depth of the object can be efficiently rendered with differentiable rasterization \cite{laine2020modular}. 
The geometry generation loss function is defined as:
\begin{align}
    \label{eq:sds_geo}
    \mathcal{L}_\text{Geo} = \lambda_\text{SD} \mathcal{L}_{\text{SDS}-\text{Normal}}^\text{SD} + \lambda_\text{ND} \mathcal{L}_{\text{SDS}-\text{ND}}^\text{ND},
\end{align}
where the first loss term is utilized in Fantasia3D \cite{chen2023fantasia3d} to imposes SDS on the rendered normal maps with Stable Diffusion, while the second loss term is enabled by our Normal-Depth diffusion model to impose SDS on the composite of the rendered normal and depth maps.

For the NeRF representation, we use the same loss function as in \eref{eq:sds_geo} by rendering normal and depth maps via volume rendering.
Given that the normal and depth maps derived from NeRF can be noisy at the start of the optimization, we impose SDS loss on the rendered RGB images with SD during the first 1,000 iterations to warm up the optimization.

\paragraph{Appearance Modeling}
The second step in our pipeline involves the synthesis of appearance.
For DMTet representation, in line with prior studies \cite{chen2023fantasia3d,Munkberg_2022_CVPR}, we employ the Physically Based Rendering (PBR) Disney material model \cite{burley2012physically}, which integrates a diffuse term with a specular GGX lobe \cite{walter2007microfacet}.
The material property of a surface point is determined by the diffuse color $\diffuse \in \real^3$, roughness $\roughness \in \real$, metallic term $\metallic \in \real$, and normal variation in tangent space $\ntangent \in \real^3$. 
We parameterize the spatially-varying materials of the surface by a learnable MLP $\mlpmaterial$ with parameters $\parammat$ to predict material parameters for input 3D point $p$ as:
\begin{align}
    \label{eq:}
    (\diffuse, \roughness, \metallic, \ntangent) = \mlpmaterial (p).
\end{align}
By specifying the environment lighting and the camera viewpoint, the image color can be computed using a differentiable renderer based on the surface geometry and materials \cite{Munkberg_2022_CVPR}.

The existing method optimizes the materials by imposing SDS loss on the final rendered RGB images \cite{chen2023fantasia3d}.
This approach, however, may lead to material decomposition inaccuracies due to the inherent challenges in disentangling material components based solely on color. To circumvent this limitation, we integrate our Albedo diffusion model to apply an additional SDS loss on the albedo component, thus enhancing the regularity of the decomposition process. The appearance modeling loss function is expressed as:
\begin{align}
    \label{eq:sds_app}
    \mathcal{L}_\text{App} = \lambda_\text{SD}' \mathcal{L}_{\text{SDS}-\text{RGB}}^\text{SD} + \lambda_\text{Albedo}' \mathcal{L}_{\text{SDS}-\text{Albedo}}^\text{Albedo},
\end{align}
where the first term reflects the SDS on the rendered RGB images using SD, and the latter term is the SDS imposed on the albedo component by our Albedo diffusion model.

After optimization, the material properties can be sampled at surface points and compiled into a 2D texture map \cite{chen2023fantasia3d,Munkberg_2022_CVPR,xatlas}, which can be directly imported into existing graphics engines for applications.

\paragraph{Optimization}
For geometry generation, 
we represent the scene with a hashgrid representation \cite{muller2022instant} \todo{model architecture}.
The loss weights $\lambda_\text{SD}$ and $\lambda_\text{ND}$ are both set to $1$. The optimization process takes approximately $1.5$ hours on a single GPU with $30$ GB of memory for both NeRF and DMTet.

For appearance modeling, the loss weights $\lambda_\text{SD}'$ and $\lambda_\text{ND}'$ are also set to $1$.
\todo{More details, e.g., CFG rescaling}

%\section{Preliminary}
%
%\subsection{Diffusion Model for Text-to-Image}
%Diffusion models have achieved great successes in text-to-image synthesis\cite{rombach2022high,ramesh2022hierarchical}, by systematically inject noise $\epsilon$ into a data sample $x$ and iteratively reverse this noising to perform denoising \cite{ho2020denoising,sohl2015deep}. The objective minimized in this process is given by:
%\begin{align}
%    \mathcal{L}_{\text{DM}} = \mathbb{E}_{\data, \noise \sim \mathcal{N}(0,1)}\left[\|\noise_{\dmparam}(\data_\dmtime, \dmtime) - \noise\|^2_2\right],
%\end{align}
%where $\data_\dmtime = \sqrt{\bar{\alpha}_\dmtime}\data + \sqrt{1 - \bar{\alpha}_\dmtime}\noise$ is the noised data variable at a specific denoising timestep $\dmtime$,
%and $\noise_{\phi}(\data_\dmtime, t)$ denotes the noise prediction function parameterized by a UNet-based network. The term $\bar{\alpha}_t$ indicates the variance schedule that regulates the level of noise at each denoising step.
%
%\subsection{Score Distillation Sampling}
%Let the function describing the Neural Radiance Fields (NeRF) rendering be denoted by $\image=\volumerender(\nerfparam)$, with $\image$ representing the output image, and $\nerfparam$ signifying the parameters of the NeRF model. Based on the innovations by Poole et al.~\cite{poole2022dreamfusion}, Score Distillation Sampling (SDS) is a technique that leverages gradient-based score functions to steer the optimization of NeRF parameters for the synthesis of 3D objects:
%\begin{equation}
%    \label{eq:sds}
%    \nabla_{\nerfparam} \mathcal{L}_{\text{SDS}}(\phi, \image=\volumerender(\nerfparam)) = \mathbb{E}_{\dmtime, \noise}\left[w(t)(\noise_{\phi}(\latent_\dmtime ; \prompt, \dmtime) - \noise) \frac{\partial \image}{\partial \nerfparam}\right],
%\end{equation}
%in which the expression $(\noise_{\phi}(\latent_t; \prompt, t) - \noise)$ represents the discrepancy between the actual noise $\noise$ and the noise estimated by the UNet $\noise_{\phi}$. The function $w(t)$ is a weighting term that is functionally dependent on the timestep $t$, and $\prompt$ embodies the text embedding obtained from the CLIP model \cite{radford2021learning}.



%The physically-based rendering (PBR) material model consists of a diffuse component (parameterized by the albedo) and a specular component (determined by the metallic and roughness parameters) \cite{burley2012physically}. 
%An ideal prior model for appearance modeling should be able to regularize both components.
%However, due to the diverse creation methods and lack of standardization of existing 3D models, it is difficult to obtain a large-scale dataset with consistent ground-truth metallic and roughness data.
%To enhance the quality of material generation, we propose an albedo diffusion model to decouple the albedo from the intricate lighting effects, serving as a preliminary approach to mitigate the challenge of mixed illumination. 



==> tables/equations.tex <==
\newcommand{\normal}{\boldsymbol{n}}
\newcommand{\point}{\boldsymbol{x}}

%\resizebox{0.48\textwidth}{!}{
    %\large
\renewcommand{\arraystretch}{1.3}
    \begin{tabular}{llll}
        \toprule
        Notation & Example\\
        \midrule
         Fraction &  $\frac{1}{a}$ \\
         Max & $\max (a, 0 )$ \\
         Dimension & $\boldsymbol{x} \in \mathbb{R}^3$ \\
         Argmax  & $\mathop{\arg\max}_{a} f(ax)$ \\
         cos & $\cos(x)$ \\
         Hat/tilde & $\hat{\boldsymbol{x}}, \tilde{\boldsymbol{x}}$ \\
         Tensor operation & $\otimes$, \quad $\circ$, \quad $\odot$ \\ 
         Sum & $\sum_{i=1}^{N} x_i$ \\
         Approximation & $f(x) \approx g(x)$ \\
         Around & $\sim$100 \\
         Product & $\prod_{i=1}^{N} x_i$ \\
         Integral & $\int_{-\infty}^{+\infty} x_i$ \\
         Gradient & $\boldsymbol{n}(n) = \nabla o(\boldsymbol{x})/\|\nabla o(\boldsymbol{x})\|_2$ \\
         Parallel & $\mathcal{L} = \sum \| x_i - \hat{x}_i \|^2_2$ \\
         Set & $\{I_i | i=1,\dots, N \}$ \\
        \bottomrule
    \end{tabular}
%    }



==> tables/greek_letters.tex <==
    \resizebox{0.48\textwidth}{!}{
    \large
    \begin{tabular}{clclclclc}
        \toprule
        Symbol & \LaTeX  & Symbol & \LaTeX & Symbol & \LaTeX\\
        \midrule
$\alpha  $ & \textbackslash alpha   & $\kappa $ & \textbackslash kappa  & $\psi    $  & \textbackslash psi    \\
$\beta   $ & \textbackslash beta    & $\lambda$ & \textbackslash lambda & $\rho    $  & \textbackslash rho    \\
$\chi    $ & \textbackslash chi     & $\mu    $ & \textbackslash mu     & $\sigma  $  & \textbackslash sigma  \\
$\delta  $ & \textbackslash delta   & $\nu    $ & \textbackslash nu     & $\tau    $  & \textbackslash tau    \\
$\epsilon$ & \textbackslash epsilon & $ o     $ & \textbackslash o      & $\theta  $  & \textbackslash theta  \\
$\eta    $ & \textbackslash eta     & $\omega $ & \textbackslash omega  & $\upsilon$  & \textbackslash upsilon\\
$\gamma  $ & \textbackslash gamma   & $\phi   $ & \textbackslash phi    & $\xi     $  & \textbackslash xi     \\
$\iota   $ & \textbackslash iota    & $\pi    $ & \textbackslash pi     & $\zeta   $  & \textbackslash zeta   \\
\midrule
$ \digamma   $ & \textbackslash digamma    & $ \Delta $ & \textbackslash digamma    & $ \Theta   $  & \textbackslash Theta  \\
$ \varepsilon$ & \textbackslash varepsilon & $ \Gamma $ & \textbackslash varepsilon & $ \Upsilon $  & \textbackslash Upsilon\\
$ \varkappa  $ & \textbackslash varkappa   & $ \Lambda$ & \textbackslash varkappa   & $ \Xi      $  & \textbackslash Xi     \\
$ \varphi    $ & \textbackslash varphi     & $ \Omega $ & \textbackslash varphi     &               &         \\
$ \varpi     $ & \textbackslash varpi      & $ \Phi   $ & \textbackslash varpi      & $ \aleph   $  & \textbackslash aleph  \\
$ \varrho    $ & \textbackslash varrho     & $ \Pi    $ & \textbackslash varrho     & $ \beth    $  & \textbackslash beth   \\
$ \varsigma  $ & \textbackslash varsigma   & $ \Psi   $ & \textbackslash varsigma   & $ \daleth  $  & \textbackslash daleth \\
$ \vartheta  $ & \textbackslash vartheta   & $ \Sigma $ & \textbackslash vartheta   & $ \gimel   $  & \textbackslash gimel  \\
        \bottomrule
    \end{tabular}
    }



==> tables/two_subtables.tex <==
\newcommand{\PSNRT}{PSNR\xspace}
\newcommand{\VQM}{HDR-VQM\xspace}
\newcommand{\VDP}{HDR-VDP2\xspace}
\newcommand{\LowExposure}{Low-Exposure\xspace}
\newcommand{\MiddleExposure}{Middle-Exposure\xspace}
\newcommand{\HighExposure}{High-Exposure\xspace}
\newcommand{\AllExposure}{All-Exposure\xspace}

\makebox[\textwidth]{\small (a) Results on dataset A.} 
\resizebox{\textwidth}{!}{
    \Large
\begin{tabular}{l||*{2}{c}|*{2}{c}|*{3}{c}||*{2}{c}|*{2}{c}|*{2}{c}|*{3}{c}}
    \toprule
    & \multicolumn{7}{c||}{2-Exposure} & \multicolumn{9}{c}{3-Exposure} \\
    & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c||}{\AllExposure} & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\MiddleExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c}{\AllExposure} \\
    Method & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \VQM & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \PSNRT & \VDP & \VQM \\
    \midrule
    Method A & \Scnd{40.00} & 73.70 & \Scnd{40.04} & \Scnd{70.08} & \Scnd{40.02} & 71.89 & \Scnd{76.22} 
                  & \Scnd{39.61} & 73.24 & \Frst{39.67} & \Frst{73.24} & \Frst{40.01} & 67.90 & \Frst{39.77} & 70.37 & 79.55 \\
    Method B      & 34.54 & 80.22 & 39.25 & 65.96 & 36.90 & 73.09 & 65.33 
                  & 36.51 & 77.78 & 37.45 & 69.79 & 39.02 & 64.57 & 37.66 & 70.71 & 70.13 \\
    Method C  & 39.79 & \Scnd{81.02} & 39.96 & 67.25 & 39.88 & \Scnd{74.13} & 73.84 
                  & 39.48 & \Scnd{78.13} & 38.43 & 70.08 & 39.60 & \Scnd{67.94} & 39.17 & \Scnd{72.05} & \Scnd{80.70} \\
    Ours          & \Frst{41.95} & \Frst{81.03} & \Frst{40.41} & \Frst{71.27} & \Frst{41.18} & \Frst{76.15} & \Frst{78.84}
                  & \Frst{40.00} & \Frst{78.66} & \Scnd{39.27} & \Scnd{73.10} & \Scnd{39.99} & \Frst{69.99} & \Scnd{39.75} & \Frst{73.92} & \Frst{82.87} \\
    \bottomrule
\end{tabular}
}

\vspace{0.5em}
\makebox[\textwidth]{\small (b) Results on dataset B.} 
\resizebox{\textwidth}{!}{
    \Large
\begin{tabular}{l||*{2}{c}|*{2}{c}|*{3}{c}||*{2}{c}|*{2}{c}|*{2}{c}|*{3}{c}}
    \toprule
    & \multicolumn{7}{c||}{2-Exposure} & \multicolumn{9}{c}{3-Exposure} \\
    & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c||}{\AllExposure} & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\MiddleExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c}{\AllExposure} \\
    Method & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \VQM & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \PSNRT & \VDP & \VQM \\
    \midrule
    Method A & 37.73 & 74.05 & 45.71 & 66.67 & 41.72 & 70.36 & 85.33 
                  & 37.53 & 72.03 & 36.38 & 65.37 & 34.73 & 62.24 & 36.21 & 66.55 & 84.43 \\
    Method B      & 36.41 & 85.68 & \Scnd{49.89} & \Scnd{69.90} & 43.15 & 77.79 & 78.92 
                  & 36.43 & 77.74 & 39.80 & \Scnd{67.88} & \Scnd{43.03} & \Scnd{64.74} & 39.75 & \Scnd{70.12} & 87.93 \\
    Method C  & \Scnd{39.94} & \Scnd{86.77} & 49.49 & 69.04 & \Scnd{44.72} & \Scnd{77.91} & \Scnd{87.16} 
                  & \Scnd{38.34} & \Scnd{78.04} & \Scnd{41.21} & 66.07 & 42.66 & 64.01 & \Scnd{40.74} & 69.37 & \Scnd{89.36}\\
    Ours          & \Frst{40.83} & \Frst{86.84} & \Frst{50.10} & \Frst{71.33} & \Frst{45.46} & \Frst{79.09} & \Frst{87.40} 
                  & \Frst{38.77} & \Frst{78.11} & \Frst{41.47} & \Frst{68.49} & \Frst{43.24} & \Frst{65.08} & \Frst{41.16} & \Frst{70.56} & \Frst{89.56}\\
    \bottomrule
\end{tabular}
}

